Rayleigh-Plateau Instability on an angled and eccentric fiber: An alternative approach

This research explores the modulation of Rayleigh-Plateau instability by adjusting the orientation angle and eccentricity of a wire within a nozzle. We demonstrate that both the angle and eccentricity significantly influence the Rayleigh-Plateau instability regimes. They both also influence characteristics, such as bead velocity along the wire, bead spacing (wavelength), and bead volume. Notably, when wires are both angled and eccentric, the effect of angle prevails. Our approach includes an empirical scaling analysis, comparing gravity, curvature-induced force, and viscosity forces on a single bead, yielding a unified empirical viscous force law, and enhancing understanding of Rayleigh-Plateau regime dynamics. This new framework enriches our understanding of the forces at play in Rayleigh-Plateau instability and provides practical insights into the manipulation of fluid dynamics in industrial applications.

==> add.tex <==
% \documentclass{article}
    
% \usepackage{subfiles}
% \usepackage{titling}  % if you need separate title pages for the subfiles

% \begin{filecontents}{main_prf_drop_on_wire.tex}
% \end{filecontents}


% \begin{filecontents}{supplementary_prf_drop_on_wire.tex}
% \end{filecontents}
% % The actual document that combines both of the above documents ignoring their preambles:

% \begin{document}

% \subfile{main_prf_drop_on_wire}

% \subfile{supplementary_prf_drop_on_wire}

% \end{document}
\begin{document}

\include{supplementary_prf_drop_on_wire.tex}
\include{main_prf_drop_on_wire.tex}
\end{document}
